LTM3D: Bridging Token Spaces for Conditional 3D Generation with Auto-Regressive Diffusion Framework

We present LTM3D, a Latent Token space Modeling framework for conditional 3D shape generation that integrates the strengths of diffusion and auto-regressive (AR) models. While diffusion-based methods effectively model continuous latent spaces and AR models excel at capturing inter-token dependencies, combining these paradigms for 3D shape generation remains a challenge. To address this, LTM3D features a Conditional Distribution Modeling backbone, leveraging a masked autoencoder and a diffusion model to enhance token dependency learning. Additionally, we introduce Prefix Learning, which aligns condition tokens with shape latent tokens during generation, improving flexibility across modalities. We further propose a Latent Token Reconstruction module with Reconstruction-Guided Sampling to reduce uncertainty and enhance structural fidelity in generated shapes. Our approach operates in token space, enabling support for multiple 3D representations, including signed distance fields, point clouds, meshes, and 3D Gaussian Splatting. Extensive experiments on image- and text-conditioned shape generation tasks demonstrate that LTM3D outperforms existing methods in prompt fidelity and structural accuracy while offering a generalizable framework for multi-modal, multi-representation 3D generation.

==> Chapters/method_kx.tex <==

\section{Method} \label{section:method}

We propose a conditional 3D shape generation framework to generate shape tokens in latent space across various 3D representations with multiple input conditions. As shown in Fig.~\ref{fig:pipeline}, our framework comprises three main components, which are described in the following sections.
% \cxj{Fig. 2 has 5 subfigures, which would correspond to five components from my point of view. But when you say three main components, it is confusing how they correspond to each other. Also, it is not clear to me how Fig. 2 shows the key idea of realizing the "unified framework" for generation. }
% In Section~\ref{method:uni_latent_rep}, we describe how various 3D representations are mapped into a unified format represented by latent tokens. Section~\ref{method:cond_shape_gen} describes our conditional shape generation network, which encodes text or image inputs as conditional tokens and models the token sequence distribution through a diffusion process in an auto-regressive manner. Finally, in Section~\ref{method:recon_guide_sampling}, we present our reconstruction guided sampling strategy, which uses reconstructed latent tokens as priors to generate more faithful samples.

\subsection{Condition Adapter}

Existing conditional generation methods~\cite{li2024autoregressive, zhang20233dshape2vecset, zhang2024clay} often directly use image or text tokens as conditions, but the inherent latent space domain gap may hamper the generation faithfulness between the conditions and generated shapes, as illustrated in Michelangelo~\cite{zhao2024michelangelo}. To address this, we design a Condition Adapter module that generates prefix tokens by projecting input condition tokens.
Given an input image or a text description, we first encode them as condition tokens  $\bm{C}$.
Specifically, we encode input image via a pre-trained DinoV2~\cite{oquab2023dinov2} and encode input text description using a pre-trained CLIP~\cite{radford2021learning} model. We then initialize a set of learnable tokens, $\bm{Q} = \{\bm{q}_1, \dots, \bm{q}_k\}$, as the network parameters. 
Through a cross-attention layer and a feed-forward layer, we generate prefix tokens $\bm{T}$ by integrating semantic information from condition tokens$\bm{C}$. This process can be formulated as
\begin{equation}
\bm{T} = {\rm FF}({\rm CrossAttn}(\bm{Q}, \bm{C}) + \bm{Q}).
\end{equation}

Aligning condition tokens to the shape domain can help ensure more seamless conditioning, which improves the consistency of generated shapes with their prompts. 
Additionally, using prefix learning allows us to generalize conditions across diverse prompt types (image and text) while maintaining compatibility within the 3D shape generation framework. This results in a model capable of generating accurate shapes across diverse 3D representations, while also improving faithfulness to prompts and adaptability to various multi-modal input conditions.

\subsection{Latent Token space Modeling backbone}

% \subsection{Pre-processing and Post-processing} \label{method:uni_latent_rep}

Our latent token space modeling backbone, LTM3D, is built on the shape latent space.
To obtain latent representations, we first pre-process various 3D data formats (e.g., SDF, mesh, point cloud, or 3DGS) using their respective auto-encoder models, each with an encoder $f_{enc}$ and a decoder $f_{dec}$. Given 3D shape $S$, we apply $f_{enc}(S)$ to obtain its latent representation, typically a set of vectors, which is then flattened into shape tokens, $\{\bm{x}_1, \dots, \bm{x}_n\}$, denoted as $\bm{X} \in \mathbb{R}^{n \times d}$. 
Following MAR's~\cite{li2024autoregressive} auto-regressive diffusion framework, LTM3D aims to model the conditional shape distribution $p(\bm{X}|\bm{C})$ given image or text prompts $\bm{C}$. 
The LTM3D backbone is composed of a Masked Auto-Encoder network for learning inter-token dependencies and a MLP-based DenoiseNet for learning conditional token distributions.
% Built on the MAR~\cite{li2024autoregressive} model, Uni3DGen consists of three core components: \textit{prefix learning}, \textit{inter-token dependency learning} and \textit{next-token distribution modeling}.
% \cxj{Better to have clear correspondence between the names of these components and the module names in the figures. }

% \noindent
% \textbf{Prefix Learning.} 


% \noindent \textbf{Inter-token Dependency Learning.} 
To exploit inter-token dependencies between prefix tokens and shape tokens, previous methods~\cite{zhao2024michelangelo, zhang20233dshape2vecset, zhang2024gaussiancube,zhang2024clay} learn the conditional joint distribution by minimizing an objective formulated as $\text{D}(q(\bm{X}|\bm{T}), p(\bm{X}|\bm{T}))$, where $q(\bm{X}|\bm{T})$ is the estimated distribution and $\text{D}(\cdot,\cdot)$ denotes a distance function between two distributions. However, as sequence length increases, optimizing this joint distribution becomes increasingly challenging due to the exponential complexity of inter-token dependencies, which may hinder capturing intricate details in shape latent tokens.
As demonstrated in MAR~\cite{li2024autoregressive}, decomposing the inter-token dependency learning part from the optimization target can help reduce optimization complexity.
We follow MAR to decompose the joint distribution into a product of conditional distributions, expressed as $\prod_{i=1}^n p(\bm{x}_i | \bm{x}_{<i}, \bm{T})$, reformulating the optimization objective as 
\begin{equation}
\text{min} \sum_{i=1}^n \text{D}(q(\bm{x}_i | \bm{x}_{<i}, \bm{T}), p(\bm{x}_i | \bm{x}_{<i}, \bm{T})).
\end{equation}

To optimize this objective, we follow MAR to approximate $q(\bm{x}_i | \bm{x}_{<i}, \bm{T})$ as $q(\bm{x}_i | \bm{z}_i)$, where $\bm{z}_i=f(\bm{x}_{<i}, \bm{T})$ represents the dependencies between $\bm{x}_i$ and $\bm{x}_{<i}, \bm{T}$. 
As shown in Fig.~\ref{fig:pipeline}, a Masked Auto-encoder (MAE) is employed to learn inter-token dependencies as $\bm{z}_i=\text{MAE}(\bm{x}_{<i}, \bm{T})$.
% \cxj{Is it helpful to mark these symbols in the figure?}

% \noindent
% \textbf{Next-token Distribution Modeling.} 
Our approach diverges from traditional diffusion methods that model $p(\bm{X}|\bm{T})$ as a joint distribution, which can be challenging to optimize for complex 3D data. Instead, we adopt the decomposition strategy used in MAR~\cite{li2024autoregressive}, where the factorized conditional distribution $p(\bm{x}_i|\bm{z}_i)$ is independently modeled through a DenoiseNet.
We employ the same objective function for DenoiseNet as MAR, formulated as:
\begin{equation} \label{eq:diff_loss}
\mathcal{L}(\bm{x}_i, \bm{z}_i) = \mathbb{E}_{\epsilon, t}[\Vert \epsilon - \epsilon_\theta(\bm{x}_i|t,\bm{z}_i) \Vert^2], \end{equation}
where $\epsilon$ is a noise token sampled from $\mathcal{N}(\bm{0}, \bm{I})$, $t$ represents the time step, and $\epsilon_\theta$ denotes the predicted noise token from the DenoiseNet parameterized by $\theta$. This factorized diffusion approach refines each token iteratively based on its inter-token dependencies, allowing for more accurate modeling of intricate 3D shapes.
% \cxj{This factorization is not clearly illustrated in Fig 2 (c). Can we show the independency in the figure?}

% \cxj{Are the CA, FF, MAE, and DenoiseNet modules in Fig 2(b)(c) trained together? }

\subsection{Reconstruction Adapter} \label{method:recon_guide_sampling}

During the generation, we auto-regressively sample shape tokens for shape decoding.
In this process, the probabilistic distribution of the first several tokens, $p(\bm{x}_i|\bm{x}_{<i},\bm{T})$, often lacks determinism due to limited conditioning information, potentially leading to diverse sampled shapes that are not faithful to the input prompts. 
%We propose a \textit{Reconstruction Guided Sampling} mechanism, as shown in Fig.~\ref{fig:pipeline} (e), 
To ensure accurate generated shapes aligned with the input conditions, we design a \textit{Reconstruction Adapter} module that reconstructs shape tokens from the condition tokens, as illustrated Fig.~\ref{fig:pipeline}. 
This module comprises a cross-attention layer followed by $D$ self-attention blocks.
We first initialize a set of learnable tokens $\bm{Q}^S$ as the optimizable parameters, then generate reconstructed tokens $\bm{\hat{X}}$ following
\begin{equation}
\bm{\hat{X}} = {\rm SelfAttn}({\rm CrossAttn}(\bm{Q}^S, \bm{C}) + \bm{Q}^S).
\end{equation}

%\cxj{From the learnable "initial" tokens? So how to produce these learnable tokens from the condition?}
% Building on this, we introduce a reconstruction guided sampling strategy, shown in Fig.~\ref{fig:pipeline} (e). 
Given the reconstructed tokens $\bm{\hat{x}}_{<i}$ alongside the diffusion-sampled tokens $\bm{x}_{<i}^S$, we blend them through a linear combination weighted by $\alpha_i$, formulating the input sequence $\bm{x}_{<i}^F$ for the MAE network. The process for sampling the next token is formulated as:
\begin{equation} 
\begin{split}
\bm{x}_{<i}^F&=(1-\alpha_i)\cdot\bm{\hat{x}}_{<i}+\alpha_i\cdot\bm{x}_{<i}^S, \\
\bm{z}_i&={\rm MAE}(\bm{x}_{<i}^F), \\
\bm{x}_i^S&={\rm Sample}(\bm{z}_i).
\end{split}
\end{equation}

By incorporating guidance from reconstructed tokens, the condition vector $\bm{z}_i$ can leverage more accurate blended tokens $\bm{x}_{<i}^F$, effectively reducing sampling uncertainty and enhancing shape alignment with input conditions.


% We incorporate learnable positional embeddings to establish the sequence order of the flattened data, ensuring that the flattening pattern does not impact training or sampling. During generation, we obtain different 3D shape representations by post-processing the sampled latent tokens $\{\bm{x}_1^S, \dots, \bm{x}_n^S\}$ through $f_{dec}$.
% The pre-processing and post-processing operations are fundamental to support a unified generation framework for different shape latent spaces.
% By transforming various 3D representations into token sequences, we can frame the shape generation task as a general sequence distribution modeling problem, defined by
% \begin{equation}
% \text{min}~\text{D}(q(\bm{X}), p(\bm{X})),
% \end{equation}
% where $\text{D}(\cdot,\cdot)$ represents a distance function between two distributions, and $q(\bm{X})$ is the estimated distribution.

% the order does not influence the learning.

% \subsection{Conditional Shape Distribution Modeling} \label{method:cond_shape_gen}
